Ambrosia: Reduction in Data Transfer from Sensor to Server for Increased Lifetime of IoT Sensor Nodes

Data transmission accounts for significant energy consumption in wireless sensor networks where streaming data is generatedby the sensors. This impedes their use in many settings, including livestock monitoring over large pastures (which formsour target application). We present Ambrosia, a lightweight protocol that utilizes a window-based timeseries forecastingmechanism for data reduction. Ambrosia employs a configurable error threshold to ensure that the accuracy of end applicationsis unaffected by the data transfer reduction. Experimental evaluations using LoRa and BLE on a real livestock monitoringdeployment demonstrate 60% reduction in data transmission and a 2X increase in battery lifetime.

==> sec_discussion.tex <==

\section{Discussion}
\label{sec:discussion}

\begin{itemize}
    
    
    \item Comparison of different network communication technologies
    
    \item Comparison of different kind of applications. Error Threshold would depend on the type of application, e.g., for anomaly detection, we can have a high error threshold. 
    Pedometer step counting: may be okay to have a medium value of error threshold. 
    Sensor readings related to health devices: e.g., accelerometer readings to determine the location of medical monitoring devices: should have almost zero error threshold.

    \item discussion of imagery (would be exciting to extend the algorithm for the imagery case), think of real-time applications with the imagery data.




\end{itemize}



